On the Reinhardt Conjecture and Formal Foundations of Optimal Control

We describe a reformulation (following Hales (2017)) of a 1934 conjecture of Reinhardt on pessimal packings of convex domains in the plane as a problem in optimal control theory. Several structural results of this problem including its Hamiltonian structure and Lax pair formalism are presented. General solutions of this problem for constant control are presented and are used to prove that the Pontryagin extremals of the control problem are constrained to lie in a compact domain of the state space. We further describe the structure of the control problem near its singular locus, and prove that we recover the Pontryagin system of the multi-dimensional Fuller optimal control problem (with two dimensional control) in this case. We show how this system admits logarithmic spiral trajectories when the control set is the circumscribing disk of the 2-simplex with the associated control performing an infinite number of rotations on the boundary of the disk in finite time. We also describe formalization projects in foundational optimal control viz., model-based and model-free Reinforcement Learning theory. Key ingredients which make these formalization novel viz., the Giry monad and contraction coinduction are considered and some applications are discussed.

==> changelog.tex <==
\section{CHANGELOG}
\begin{itemize}
    \item \textbf{April 15, 2022} : First draft with introduction and Chapter III consisting of the formalization of model-based and model-free RL.
    \item \textbf{May 20, 2022} : Adds a significant chunk of Chapter II, including introduction and background results in discrete geometry to the statement of the Reinhardt conjecture and its gradual reduction to a problem in optimal control (See Problems \ref{pbm:reinhardt-conjecture},
    % \ref{pbm:reinhardt-conjecture-affine},
    \ref{pbm:reinhardt-reduction},\ref{pbm:reinhardt-reduction-2},\ref{pbm:plane-optimal-control-problem},\ref{pbm:reinhardt-optimal-control},\ref{pbm:state-costate-reinhardt}). The Hamiltonian (See Section \ref{sec:max-ham}), the state equations (See Section \ref{sec:lie-group-dynamics} and Section \ref{sec:lie-algebra-dynamics}), the costate equations (see Sections \ref{sec:costate-variables}) in both coadjoint orbit and half-plane pictures are derived simultaneously. Lax pair form of $X$ (see Theorem \ref{thm:X-dynamics-sl2}) and the general solution for $\Lambda_1$ (see Corollary \ref{cor:lam1-gen-sol}) is given.
    Reparamterization of $X$ is proven to be Lipschitz in Proposition \ref{prop:reparam-lipschitz}. Compactification result is written down in Section \ref{sec:compactification} and used in Filippov's theorem in Section \ref{sec:existence-opt-control}. The PMP is written down (see Section \ref{sec:PMP}) and general solutions for constant-control are written down. 
    Transversality conditions are discussed for the state and costate variables in Section \ref{sec:X-init-term-conds} and Section \ref{sec:transversality}.
    The exceptional isomorphisms of $\sl(\R)$ are discussed in Section \ref{sec:sl2-exceptional} and the Lie-Poisson dynamics for $X$ is discussed in Section \ref{sec:X-lie-poisson}.
    \item \textbf{June 6, 2022}: Added a preliminary WIP draft of the smoothed $(6k+2)$-gons in Section \ref{sec:6k+2-gons}. Also added a section on the circular control set $U_r$ (Section \ref{sec:circular-control}), together with the derivation of the angular momentum (Section \ref{sec:angular-momentum}) and using it to compute the quadratic equation for the optimal control matrix (Section \ref{sec:quadratic-equation}). A section on the control sets in $\su$ is also added (Section \ref{sec:su11-control-sets}). The control problem with the inscribed control set $U_I$ is introduced in Section \ref{sec:inscribed-control}, together with the simplifications in state, costate and the Hamiltonian. These are all used to prove that in this case, there are no periodic abnormal extremals in Section \ref{sec:no-abnormal-extremals}.
    \item \textbf{June 24, 2022}: Cleaned up the proof of the Valuation-Truncation argument in Theorem \ref{thm:valuation-truncation} along with a bunch of supporting results about valuations. Proved that our Fuller system is Hamiltonian, derived a Poisson bracket and showed that it arises via a symplectic structure on $\mathbb{C}^3$, mentioned that the Fuller system may be generalized and reported the general Hamiltonian and angular momentum \ref{sec:fuller-system}. Reported log-spiral solutions in Section \ref{sec:log-spiral-solutions}. Added appendices about the Kirillov 2-form in Section \ref{sec:kirillov} and Hypotrochoids in Section \ref{sec:hypotrochoids}. Added a new chapter, Chapter 4 about possible future work. 
    \item Incorporated all comments on Chapter II. Changed notation from $Z_0$ to $Z_0$ and ``convex domain'' to ``convex disc''. Fixed the Compactification proof in Section \ref{sec:compactification}. Expanded comments about the Fuller system in \ref{sec:fuller-system}. Added a list of notation. 
\end{itemize} 
